HIORE: Leveraging High-order Interactions for Unified Entity Relation Extraction

Entity relation extraction consists of two sub-tasks: entity recognition and relation extraction. Existing methods either tackle these two tasks separately or unify them with word-by-word interactions. In this paper, we propose HIORE, a new method for unified entity relation extraction. The key insight is to leverage the high-order interactions, i.e., the complex association among word pairs, which contains richer information than the first-order word-by-word interactions. For this purpose, we first devise a W-shape DNN (WNet) to capture coarse-level high-order connections. Then, we build a heuristic high-order graph and further calibrate the representations with a graph neural network (GNN). Experiments on three benchmarks (ACE04, ACE05, SciERC) show that HIORE achieves the state-of-the-art performance on relation extraction and an improvement of 1.1~1.8 F1 points over the prior best unified model.

==> figs/rel-distance.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=3in]{images/fig-rel-distance.pdf}
    \end{center}
    \vspace{-10pt}
    \caption{Relation performances (F1 score) with respect to the distance between entity pairs on the ACE05 test set. Note that we use BERT$_{\texttt{BASE}}$ as the sentence encoder.}
    \label{fig:gcn}
    \vspace{-10pt}
\end{figure}

==> tables/data-statistics.tex <==
\begin{table}[tb!]
    \centering
    \footnotesize
    \begin{tabular}{cccc}
        \toprule
        Dataset      & \#sents & \#ents(\#types) & \#rels(\#types) \\
        \midrule
        ACE04  & 8,683   & 22,519(7)       & 4,417(6)        \\
        ACE05  & 14,525  & 38,287(7)       & 7,691(6)        \\
        SciERC & 2,687   & 8,094(6)        & 5,463(7)        \\
        \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{The statistics of the adopted three datasets.}
    \label{tab:data-statistics}
    \vspace{-10pt}
\end{table}

==> tables/graph.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{llcccc}
        \toprule
        \multirow{2}{*}{\textbf{Graph Type}} & \multirow{2}{*}{\textbf{\#Layers}} & \multicolumn{2}{c}{\textbf{ACE05}} & \multicolumn{2}{c}{\textbf{SciERC}}                                 \\
        ~    & ~                              & Ent                                & Rel                                 & Ent           & Rel           \\
        \midrule
        \multirow{3}{*}{Static} & 1-layer & 87.6 & \textbf{63.1} & 69.9 & 41.6 \\
        ~ & 2-layer & 87.6 & 62.6 & \textbf{69.8} & 39.9 \\
        ~ & 3-layer & 87.5 & 62.8 & 68.9 & 39.0 \\
        \midrule
        \multirow{3}{*}{Dynamic} & 1-layer & \textbf{87.9} & 62.6 & 69.7 & \textbf{40.5} \\
        ~ & 2-layer & 87.7 & 60.1 & 69.4 & 38.0 \\
        ~ & 3-layer & 87.4 & 63.4 & 69.4 & 37.3 \\
        \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{Results (F1 score) with different settings on ACE05 and SciERC test sets. Note that we use BERT$_{\texttt{BASE}}$ on ACE05.}
    \label{tab:graph}
    \vspace{-10pt}
\end{table}

==> tables/wnet.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Network}} & \multicolumn{2}{c}{\textbf{ACE05}} & \multicolumn{2}{c}{\textbf{SciERC}}                                 \\
        ~                                  & Ent                                & Rel                                 & Ent           & Rel           \\
        \midrule
        WNet                            & \textbf{89.6}                               & \textbf{65.8}                       & \textbf{68.2} & \textbf{38.3}          \\
        \midrule
        % biaffine attention & 88.8 & 65.0 & 67.2 & 36.4  \\
        single UNet                     & \textbf{89.6}                               & 65.6                       & 66.3 & 34.6         \\ 
        two separate UNets               & 88.8                              & 63.8                       & 67.9 & 37.6          \\
        \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{Performance (F1 score) with WNet and altinatives on ACE05 and SciERC test sets. ``single UNet'' means that concatenating $\bm{V}$ and $\bm{K}$ then feed it into a single UNet. ``two separate UNets'' means that using two separate UNets for $\bm{V}$ and $\bm{K}$ inputs, respectively. 
    % Note that we use BERT$_{\texttt{BASE}}$ on ACE05.
    }
    \label{tab:wnet}
    \vspace{-10pt}
\end{table}
